Motion Guided Token Compression for Efficient Masked Video Modeling

Recent developments in Transformers have achieved notable strides in enhancing video comprehension. Nonetheless, the O($N^2$) computation complexity associated with attention mechanisms presents substantial computational hurdles when dealing with the high dimensionality of videos. This challenge becomes particularly pronounced when striving to increase the frames per second (FPS) to enhance the motion capturing capabilities. Such a pursuit is likely to introduce redundancy and exacerbate the existing computational limitations. In this paper, we initiate by showcasing the enhanced performance achieved through an escalation in the FPS rate. Additionally, we present a novel approach, Motion Guided Token Compression (MGTC), to empower Transformer models to utilize a smaller yet more representative set of tokens for comprehensive video representation. Consequently, this yields substantial reductions in computational burden and remains seamlessly adaptable to increased FPS rates. Specifically, we draw inspiration from video compression algorithms and scrutinize the variance between patches in consecutive video frames across the temporal dimension. The tokens exhibiting a disparity below a predetermined threshold are then masked. Notably, this masking strategy effectively addresses video redundancy while conserving essential information. Our experiments, conducted on widely examined video recognition datasets, Kinetics-400, UCF101 and HMDB51, demonstrate that elevating the FPS rate results in a significant top-1 accuracy score improvement of over 1.6, 1.6 and 4.0. By implementing MGTC with the masking ratio of 25\%, we further augment accuracy by 0.1 and simultaneously reduce computational costs by over 31\% on Kinetics-400. Even within a fixed computational budget, higher FPS rates paired with MGTC sustain performance gains when compared to lower FPS settings.

==> bak/bak.tex <==

% In recent years, deep learning frameworks have achieved significant improvement in video action recognition\cite{?}. Most of current methods treat the video as a three dimensional image and input all the video frames into the model. Although this strategy achieves promising performance, under a certain level of computation budget, the spatial-temporal redundancy\cite{?} presented in the videos limits the algorithms to model with higher fps and resolution, longer temporal context or to have more parameters, especially for the transformer-based models\cite{?}, which naturally suffer from a $O(N^2)$ computational cost with respect to the input sequence length. To tackle this issue, researches try to decompose the spatial and temporal dimension and then model them separately \cite{arnab2021vivit, bertasius2021spacetime}. Such methods can largely reduce the memory cost but it is then challenging to learn the joint temporal-spatial relationships. Other methods use multi-stage training to select key frames related to the action\cite{?}, which is able to reduce the cost but makes the model more complicated.

% Recently, masked video modeling has been proven effective for the representation learning task\cite{?}. By taking advantages of the structure of vanilla vision transformer (ViT), a self-supervised task is built to reconstruct the whole video with a limited number of randomly selected tokens. It shows reasonable quality of the reconstruction videos from only a small proportion of the video, indicating the existence of spatial-temporal redundancy since the information from invisible tokens can be recovered by other visible tokens. Despite of this, the randomly selecting strategy is still limited in removing the redundancy. Firstly it will inevitably keep a certain ratio of redundancy tokens since every token is masked with the same probability. The redundancy level after random masking is related with the original video content, and will becomes larger as the fps goes higher. Fig{?}. Secondly the absolute number of informative tokens will decrease if a higher mask ratio is applied, That means we will have to trade off between the performance and efficiency. Such properties limits the capacity of algorithm to model with smaller patch size, higher fps and longer temporal context, which are crucial in the action recognition task.

% To address the natural redundancy of the video, video compression algorithms \cite{inproceedings} are commonly studied and used in modern video encoding. The compression algorithms generally focus on better compressing the motion information while keeping the quality of the decoded video. The key frames and motion vectors extracted from a compressed video format could benefit different vision tasks as shown in \cite{}, but the sparsity property of the motion vectors is not fully exploited, so that the redundancy and computational cost remains a concern when applying compressed video to computer vision backbones. 

% Inspired by the video compression algorithms, we propose the Motion Guided Token Compression to address the above issues. Instead of randomly masking out tokens, which will cause both redundancy and information leakage, we apply a motion-guided masking (MGM). Firstly, we uniformly split the whole video into non-overlapping patches (or cubes when the temporal range is larger than 1), each of them is treated as a token. For each token, the mean absolute difference between the current token and the token at the same spatial position in the next frames is calculated. This difference indicates how the current token will change after one frame, thus including the motion information. Then a ratio of tokens with lower token-difference are masked out. In this way we ensure more informative tokens will be kept while the redundancy tokens being removed through this lightweight token-difference. From Fig{} we can see this motion-guided masking increases the ratio of non-redundant tokens compared with random masking and the effect is more obvious when using a higher fps. Then to further prevent from information leakage, we add a temporal range embedding to indicate the number of masked tokens before any unmasked token at the same spatial position. This range embedding is used to reflect the duration of motion, which makes up the information leakage from masking out redundant tokens.

% To summarize our contributions:

% We propose Motion Guided Token Compression, consisting of lightweight motion-guided masking and temporal range embedding, which is capable of largely removing spatial-temporal redundancy as well as keeping most of the information.

% We compare our method with random masking based based on standard masked video modeling and prove the effectiveness at both pre-training and fine-tuning stages on several public benchmarks.

% Ablation experiments are done to show the proposed method has potential to breakthrough the bottleneck of computational cost and yield to better performance by using smaller patch size and higher fps.


%%%%%%%%%%%%%%


% Apart from improving the accuracy performance, another popular research direction is to consider the running efficiency and how to remove redundant information from the video becomes a key issue. Ada3D adaptively selected 2D-CNN or 3D-CNN by a two-head selection network trained with policy gradient methods. AdaFrame adaptively selected relevant frames on a per-input basis for fast video recognition. 

% The related works in video action recognition have been a significant area of research in computer vision. Numerous studies have focused on developing robust and accurate methods for recognizing and understanding human actions in videos. One common approach is to extract spatio-temporal features from video sequences, such as optical flow, motion trajectories, or 3D convolutional neural networks (CNNs), to capture the dynamic information of actions. Another direction of research involves exploring the temporal structure of actions, such as modeling long-term dependencies using recurrent neural networks (RNNs) or attention mechanisms. Additionally, there has been a growing interest in leveraging deep learning architectures, such as two-stream networks, which combine appearance and motion information, or 3D CNNs, which directly process spatio-temporal volumes. Furthermore, researchers have explored the use of large-scale video datasets and transfer learning techniques to improve action recognition performance. Overall, the related works in video action recognition have made significant advancements in developing effective algorithms and models for accurately recognizing and understanding human actions in videos, enabling applications in areas such as surveillance, video analysis, and human-computer interaction.

%%%%%%
% The goal of masked vision modeling to learn effective vision representations by reconstructing signals from corrupted ones. 
% This methodology draws inspiration from the Masked Language Modeling task from BERT\cite{devlin-etal-2019-bert}. 
% To achieve optimal results, it is crucial to design an effective reconstruction task. The reconstructed targets can be raw pixels or derived features as explored hand in hand in recent research. In addition, the masking strategy employed in masked video modeling plays a critical role. Tube masking, proposed by VideoMAE, is an effective strategy that avoids information leakage for pre-training and has been shown to outperform other masking strategies such as frame masking and random masking. To reduce redundancy in videos and computations during fine-tuning, MAR presented the running cell masking, which was also used in VideoMAE-v2 for large-scale video pre-training. Building on these methods and video compression algorithms, we propose an innovative motion-guided masking method for compressed video tokenization.


%%%%%%%%%
% In MGTC, the value of the hyperparameter $\lambda$ is critical in determining the number of cubes that need to be masked. 
% Since videos exhibit natural diversity, we cannot use a fixed value for the threshold or compute it across the entire dataset. 
% Instead, we calculate the threshold for each individual video based on its characteristics. 
% We assume that a certain percentage of each video is redundant, and set $\lambda$ to be the cube difference value at the top $N$ percent of all cubes in that video. 
% We will explore the impact of different values of $N$ in the subsequent analysis section.

% \subsection{Temporal Range Embedding}
% % IMAGE TO BE ADDED: figure to present the range embedding we add
% % Math Equation TO BE ADDED
% In the above masking strategy, we hold the assumption that such masked cubes are duplicate with the reversed ones. However, the newly masked sequence still suffers from information leakage from the original video, which we address by applying a temporal range embedding to better indicate the frame indices that each preserved cube refers to.
% However, the model fails to identify which frames the masked cubes refer to, since the current position embedding only indicates each cube's own temporal index.
% To address this issue, we add a temporal range embedding that for each reserved cube.
% As shown in \autoref{range-emb}, besides to each cube's own temporal embedding, we also aggregate the temporal embedding of its corresponding masked neighbors. 
% This allows every cube from each frame to be able to recognize all the frames that all other cubes belong to.

% \begin{figure}[]
% \centering
% \includegraphics[scale=0.2]{figures/range-emb.jpg}
% \caption{Overview of the Range Embedding}
% \label{range-emb}
% \end{figure}


%%%%%%%%%%
% We follow the training settings from VideoMAE \cite{tong2022videomae}, for which we first do a pretrianing VideoMAE reconstruction, and then do finetuning classification on downstream tasks.
% In this paper, we do not involve MGTC in the pretraining stage, but follow the same setting in the original VideoMAE. 
% The only difference is we uses a higher FPS in the pretraining, for which, the computational cost gets increased.
% In the finetuning stage, we either use all video tokens as the same in the original setting,  or use MGTC to keep informative video cubes that are able to represent the whole video for training.
% We expect that further training with MGTC would enhance the representation of the selected video patches and accelerate the training process as well.

% Then such reserved high-quality cubes are further randomly selected to do the reconstruction task.
% Now we only use a even smaller portion but more informative cubes to reconstruct the whole video in the pretraining.
% This is more likely to avoid the copy-and-pasting in the reconstruction and help the model learn a better video representation with higher compression rate and compression quality.


%%%%%%%%%

% We experiment on two widely studied video action recognition datasets, Kinetics-400 (K400) \cite{kay2017kinetics}, and UCF101 \cite{soomro2012ucf101}.
% K400 has approximately 240k training videos and 20k validation videos, each of 10 seconds duration, covering 400 classes in total. 
% UCF101 is a smaller dataset consisting of 9.5k training videos and 3.5k validation videos. 


%%%%%%%%%%%%

% We've shown a higher fps brings up the performance gain in \autoref{overview}.
% As involving more video frames largely increases the computational cost, we compare various masking strategies that are able to address such a limitation.
% MGTC is consistently better than both the Random and Running Cell mask\cite{runningcell}. 
% Even surprisingly, the model is able to achieve a higher accuracy with a only small percentage mask.
% Experiments are made on K400 dataset, and for each fps setting, we pretrain the model for 800 epochs while all other parameters are kept the same.


% \begin{figure}[htbp]

% \centering
% \begin{subfigure}{\linewidth}
% \includegraphics[width=\linewidth]{figures/mask-fps.pdf}
% \caption{\textbf{[PLACEHOLDER]}}
% \label{fig-mask-training}
% \end{subfigure}\par\medskip
% \end{figure}


%%%%%%%%%%

% MGTC is able to address the redundancy by masking the duplicate but preserving the representative tokens, while there are also some other methods such as the simple random masking and the running cell masking \cite{runningcell} that keeps tokens from fixed positions in each frame. 
% As shown in \autoref{fig-mask}, we could see that the MGTC consistently outperforms the other two methods under various masking ratios, demonstrating its effectiveness in preserving more representative tokens.
% Also, with 10\%-20\% masking, MGTC is able to achive higher accuracy scores than using all patch tokens, while the scores from other two methods keep decreasing as we increase the masking ratio.
% This further demonstrates that MGTC is better at removing the video redundancy so that it is able to help boost the performance further, with even less computational cost.


%%%%%%%%%%%

% In \autoref{fig-mask-fps}, we compare the MGTC under different FPS settings.
% The performance score becomes higher as we increase the FPS. 
% Also, there is a huge improvement when we increase the FPS from 6 to 9, while the gain becomes smaller when we further increase it to 12. 
% In a larger FPS setting, the model reaches its maximum relative performance gain with masking ratio of 10\% while it would be 25\% for lower FPS.
% Such information is consistent with that the higher FPS indeed brings more action information so that its relative redundant percentage becomes lower.
% Also, the relative performance loss from lager FPS setting becomes smaller if we use a masking ratio of 50\%, indicating that a higher FPS brings more redundancy which could be addressed by the MGTC while bring very little influence to its performance.
